QASnowball: An Iterative Bootstrapping Framework for High-Quality Question-Answering Data Generation

Recent years have witnessed the success of question answering (QA), especially its potential to be a foundation paradigm for tackling diverse NLP tasks. However, obtaining sufficient data to build an effective and stable QA system still remains an open problem. For this problem, we introduce an iterative bootstrapping framework for QA data augmentation (named QASnowball), which can iteratively generate large-scale high-quality QA data based on a seed set of supervised examples. Specifically, QASnowball consists of three modules, an answer extractor to extract core phrases in unlabeled documents as candidate answers, a question generator to generate questions based on documents and candidate answers, and a QA data filter to filter out high-quality QA data. Moreover, QASnowball can be self-enhanced by reseeding the seed set to fine-tune itself in different iterations, leading to continual improvements in the generation quality. We conduct experiments in the high-resource English scenario and the medium-resource Chinese scenario, and the experimental results show that the data generated by QASnowball can facilitate QA models: (1) training models on the generated data achieves comparable results to using supervised data, and (2) pre-training on the generated data and fine-tuning on supervised data can achieve better performance. Our code and generated data will be released to advance further work.

==> backup/1_abstract.tex <==
\begin{abstract}

Recent years have witnessed the success of question answering (QA), especially its potential to be a foundation paradigm for tackling diverse NLP tasks.
However, obtaining sufficient data to build an effective and stable QA system still remains an open problem.
For this problem, we introduce an iterative bootstrapping framework for QA data augmentation (named Snowball-QA), which can iteratively generate large-scale high-quality QA data based on a seed set of supervised examples.
Specifically, Snowball-QA consists of three modules, an answer extractor to extract core phrases in unlabeled documents as candidate answers, a question generator to generate questions based on documents and candidate answers, and a QA-pair filter to filter out high-quality QA data.
Moreover, Snowball-QA can be self-enhanced by reseeding the seed set to fine-tune itself in different iterations, leading to continual improvements in the generation quality.
We conduct experiments on the high-resource English scenario and the medium-resource Chinese scenario, and the experimental results show that our generated data can facilitate QA models: (1) training models on the generated data achieves comparable results to using supervised data, and (2) pre-training on the generated data and fine-tuning on supervised data can achieve better performance.
Our system and data will be released to advance further work soon.

% Some analyses further show that the quality of our generated data improves with iterations, indicating the effectiveness and necessity of the snowballing process.


\end{abstract}

==> backup/2_introduction.tex <==
\section{Introduction}

Recent years have witnessed the success of question answering (QA), such as machine reading comprehension (MRC)~\cite{baradaran2022survey} and open-domain question answering (ODQA)~\cite{chen2017reading,karpukhin2020dense}. In addition to the development of QA itself, many efforts have been devoted to re-formalizing various important NLP tasks into a unified QA form to better handle these tasks, such as dialogue systems~\cite{brown2020language}, information extraction~\cite{li2019entity,li2020unified,liu2020event}, and information retrieval~\cite{brown2020language}. The great performance of the recently proposed GPT-3~\cite{brown2020language} and ChatGPT~\footnote{\url{https://openai.com/blog/chatgpt/
}} further shows the feasibility and effectiveness of using QA as the foundation to handle multiple diverse NLP tasks.

Despite the potential of QA to become a fundamental paradigm, manually obtaining sufficient data to train an effective and stable QA model is time-consuming and labor-intensive~\cite{brown2020language}. To this end, we introduce an iterative bootstrapping framework to automatically generate QA data. Different from existing QA data augmentation methods, which directly build data generators to generate large-scale data~\cite{alberti2019synthetic,lewis2021paq}, our framework iteratively generates data based on a supervised seed set. During the iterative generation process, all generated data can be used to expand the seed set and enhance the entire data generation framework, leading to continually generating data with higher quality and larger scale. \citet{agichtein2000snowball} refer to this process as snowball, and for convenience, we name our framework ``QASnowball''.

\begin{figure*}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{figs/filter.png}
    \caption{The architecture of P-PET when the number of active PET modules is 2. The working process can be split into two procedures: PET module pre-selection and prediction with active PET modules.}
    \label{fig:model-large}
\end{figure*}

QASnowball divides the entire process of generating QA data into three steps: answer extraction, question generation, and data filtering. Accordingly, QASnowball builds three core modules for these steps: an answer extractor, a question generator, and a QA data filter. All these three modules are trained based on the seed set. During the generation process, given an unlabeled document, the answer extractor is first employed to extract the core phrases in the document that are most likely to work as answers. These extracted phrases serve as answer candidates for the subsequent question generation and data filtering. Then, the question generator is used to generate a corresponding question for each answer candidate, and the QA data filter is further applied to determine whether the generated questions match the documents and the candidate answers. The well-matched question-answer pairs are combined with the document as the final generated data.

Considering that the initial seed set includes only a portion of supervised QA samples, relying exclusively on the initial seed set may make the generated data lack diversity and coverage. To avoid this issue, QASnowball adopts an iterative bootstrapping framework to generate data. Given an unlabeled corpus, instead of directly generating QA data based on the corpus at once, QASnowball divides the corpus into several pieces and generates data based on only one piece at each iteration.
After completing the generation process of each iteration, the generated data is integrated into the seed set to fine-tune the answer extractor, question generator, and data filter. Through this iterative self-enhancement mechanism, QASnowball can continually improve the quality of the generated data and make the generated data more diverse than the initial seed set.

To evaluate the effectiveness of QASnowball, we conduct experiments in both the high-resource English and medium-resource Chinese scenarios. We choose the recent competitive QA model PERT~\cite{cui2022pert} and train PERT on different datasets,  including our auto-labeled data and some existing supervised and auto-labeled datasets. By comparing the results of PERT trained on different datasets, we can evaluate the impact of these datasets on the performance of QA models. 


The experimental results show that:
\begin{itemize}
\item Training PERT only on the auto-generated data can achieve comparable results to training PERT on existing supervised datasets, indicating the high quality of the generated data. 
\item Pre-training PERT on the auto-generated data and then fine-tuning the pre-trained PERT on the supervised data can outperform using only the supervised data, demonstrating that the generated data can well supplement the supervised data. 
\item Compared with the recently proposed auto-generated data PAQ~\cite{lewis2021paq}, the data generated by QASnowball can help the QA model achieve better performance, indicating the effectiveness of the self-enhanced mechanism.
\end{itemize}
% Some empirical analyses are further conducted to reveal the relation between the data quality and the iteration mechanism in a more fine-grained manner.
% To advance the exploration of effective data augmentation methods, especially for the QA task, the code and generated data of QASnowball will be publicly available.


% We also show that SGQ is useful for training CBQA models in the few-shot tasks, and the generated QA-pairs from later iterations show higher improvements in multiple datasets. We experimented on Bert-based question-answering models such as PERT on SQUAD and CMRC2018\citep{cui-emnlp2019-cmrc2018} datasets. This demonstrates the effectiveness of SGQ and our SnowBall-QA pipeline. 

% In summary, our main contributions are threefold: 
% 1) We propose a novel pipeline for QA-pairs generation; 2) We will open-source SGQ dataset and the Snowball-QA pipeline which could be easily used for generating English or Chinese QA-pairs datasets; 3) Our experiments show that the state-of-the-art QA models could benefit from our extended data-set in multiple datasets.


\section{QASnowball}

In this section, we will introduce the details of our iterative bootstrapping framework QASnowball.

\subsection{The Overall Framework}

The overall framework of QASnowball consists of three modules: an answer extractor, a question generator, and a data filter. As shown in Figure~\ref{fig:filter}, these modules work in a pipeline to automatically generate QA data.

Specifically, given an unlabeled document $D$: 
(1) \textbf{The answer extractor} first extracts the core phrases $\mathcal{A}_D = \{A_D^1, A_D^2, \ldots, A_D^n\}$ that are most likely to be answered in $D$ as answer candidates. 
(2) \textbf{The question generator} generates the question set $\mathcal{Q}_D = \{Q_D^1, Q_D^2, \ldots, Q_D^n\}$ corresponding to the answer set $\mathcal{A}_D$, according to both the semantics of the given document and the answer candidates, where $Q_D^i$ is corresponding to $A_D^i$. 
(3) \textbf{The data filter} selects high-quality question-answer pairs from the combinations of $\mathcal{A}_D$ and $\mathcal{Q}_D$, and the selected question-answer pairs are combined with $D$ to form the final generated data.

All modules of QASnowball are first trained on the supervised seed set $\mathcal{S}$. Considering $\mathcal{S}$ cannot cover sufficient data to train all modules well, QASnowball thus iteratively generates data. At the $i$-th iteration, the newly formed data set $\mathcal{S}_i$ is used to expand the seed set and fine-tune the modules of QASnowball, and QASnowball goes over the whole process again with the fine-tuned modules in subsequent iterations. Next, we will briefly introduce the three modules of QASnowball and describe how to make the whole framework iteratively self-enhanced.

\subsection{Answer Extractor}

Given a document $D$, we treat extracting the core phrases in $D$ that are most likely to be answers as a sequence labeling problem.
For each token in $D$, we ask the extractor to determine whether the token is part of a answer candidate, and merge adjacent tokens predicted to be part of an answer to form a answer candidate.
Specifically, we adopt BERT~\cite{devlin2019bert} as the backbone model of our extractor, which is a typical auto-encoding pre-trained language model (PLM) built on the encoder architecture, and then build a binary classifier based on the backbone to identify whether each token is part of an answer. In order to facilitate the subsequent introduction of our framework, we formalize the extraction process as
\begin{equation*}
\mathcal{A}_D = \{A_D^1, A_D^2, \ldots, A_D^n\} = \texttt{EA}(D).
\end{equation*}
The extractor is first trained on the supervised seed samples, taking the documents and answers of these seed samples as supervision signals. During iterative data generation, the extractor can be improved with newly generated data.

\subsection{Question Generator}

Given a document $D$ and an answer candidate $A_D^i$ extracted from $D$, we treat generating the question $Q_D^i$ corresponding to $A_D^i$ as a contextual generation problem.
Specifically, we select T5~\cite{raffel2020exploring} as the generator backbone, which is a typical generative PLM built on the encoder-decoder architecture. 
Before generating the question, we first add special tags before and after the span of $A_D^i$ to highlight the position of the answer candidate. 
For example, given the document \textit{``... Mark Twain was born on November 30, 1835, in Florida, Missouri ...''} and the answer candidate \textit{``Florida, Missouri''}, we add two special tags (e.g., \textit{``<ANS>''} and \textit{``</ANS>''}) and then input \textit{``... Mark Twain was born on November 30, 1835, in <ANS> Florida, Missouri </ANS> ...''} into the generator. 
By feeding the tagged document into the encoder of the generator, we require the decoder of the generator to output the corresponding question. We formalize the generation process as
\begin{equation*}
\mathcal{Q}_D = \{Q_D^1, Q_D^2, \ldots, Q_D^n\} = \texttt{QG}(D, \mathcal{A}_D).
\end{equation*}
Similar to the answer extractor, the question generator is first trained on the seed set, by taking the documents and answers of seed samples as input and questions as output supervision signals. The newly generated data will also be used to fine-tune the generator, enabling the generator to generate more diverse questions beyond the domain constraints of the initial seed set.

\subsection{Data Filter}

Generally, existing methods usually train a QA model to filter the generated data~\cite{lewis2021paq}. Given a document $D$ and its candidate question-answer pair $(Q_D^i, A_D^i)$, these filtering methods adopt QA models to directly give the reasonableness score of $A_D^i$ based on the semantics of $D$ and $Q_D^i$. Based on the reasonableness scores, these filtering methods can select high-quality data. 
Although these methods have achieved promising results, the filtering quality of these methods depends heavily on the performance of the QA models, and it is difficult to select out those samples that are correctly generated but judged ambiguously by the QA models, which obviously contradicts the purpose of generating QA data to further enhance the QA model.

In this paper, we build the data filter based on the ensemble of the QA model and heuristic rules. Specifically, we choose the recent competitive QA model PERT~\cite{cui2022pert} as the backbone of the filter. Instead of giving the reasonableness score of $A_D^i$, we require the filter backbone to generate an answer $\tilde{A}_D^i$ based on $D$ and $Q_D^i$, without considering $A_D^i$. Then, several heuristic rules are adopted to select and modify the data:
\begin{itemize}
\item if $A_D^i$ does not overlap with $\tilde{A}_D^i$ any more, we discard this example.
\item if $A_D^i$ matches $\tilde{A}_D^i$ exactly, the example $\big(D, Q_D^i, A_D^i\big)$ is finally generated.
\item If $A_D^i$ partially overlaps with $\tilde{A}_D^i$, the example of $\big(D, Q_D^i, [A_D^i; \tilde{A}_D^i]\big)$ is finally generated, where $[A_D^i; \tilde{A}_D^i]$ denotes the combination of $A$ and $\tilde{D}$, such as combining \textit{``Florida,''} and \textit{``Missouri''} into \textit{``Florida, Missouri''}.
\end{itemize}
For convenience, we formalize the filtering as
\begin{equation*}
\mathcal{G}_D = \texttt{F}(D, \mathcal{A}_D, \mathcal{Q}_D),
\end{equation*}
where $\mathcal{G}_D$ is the final generated example set. Compared with the existing filtering methods based entirely on QA models, our filter not only ensures the data quality, but also retains some generated data inconsistent with QA models, which can bring better data diversity. 

\begin{algorithm}[t]
    \caption{The iterative generation process of QASnowball}
    \label{alg:AOA}
    \renewcommand{\algorithmicrequire}{\textbf{Input:}}
    \renewcommand{\algorithmicensure}{\textbf{Output:}}
    \begin{algorithmic}[1]
        \REQUIRE The seed set $\mathcal{S}$, the unlabeled document set $\mathcal{D}$, and the iteration number $t$
        \STATE  Divide the unlabeled document set into several parts according to $t$, and obtain $\mathcal{D}_{1}, \mathcal{D}_{2}, \ldots, \mathcal{D}_{t}$
        \FOR{$i \in [1, t]$}
            \IF{$i = 1$}
                \STATE Train the extractor $\texttt{AE}$, the generator $\texttt{QG}$, and the filter $\texttt{F}$ with $\mathcal{S}$
            \ELSE
                \STATE Fine-tune the extractor $\texttt{AE}$, the generator $\texttt{QG}$, and the filter $\texttt{F}$ with $\mathcal{S}$
            \ENDIF
            % \STATE Define the generated data set of the $i$-th iteration 
            \STATE $\mathcal{S}_i \leftarrow \emptyset$
            \FOR{$D \in \mathcal{D}_{i}$}
                \STATE $\mathcal{A}_D \leftarrow  \texttt{AE}(D)$
                \STATE $\mathcal{Q}_D \leftarrow  \texttt{QG}(D, \mathcal{A}_D)$
                \STATE $\mathcal{G}_D \leftarrow  \texttt{F}(D, \mathcal{A}_D, \mathcal{Q}_D)$
                \STATE $\mathcal{S}_i \leftarrow \mathcal{S}_i \cup \mathcal{G}_D$
            \ENDFOR
            \STATE Update $\mathcal{S}$ with $\mathcal{S}_i$
        \ENDFOR
        \ENSURE The generated data of all iterations $\mathcal{S}_1$, $\mathcal{S}_2$, $\ldots$, $\mathcal{S}_t$, the answer extractor $\texttt{AE}$, the question generator $\texttt{QG}$, the data filter $\texttt{F}$.
    \end{algorithmic}
\end{algorithm}


\subsection{Iterative Bootstrapping Process}

As we mentioned before, using only the initial supervised seed set to build the generation system and generate data at once may suffer from diversity and coverage issues. Therefore, QASnowball takes an iterative approach to generate data and dynamically fine-tunes the QASnowball framework during the generation process.
Specifically, given an unlabeled document set $\mathcal{D}$ that requires QASnowball to annotate questions and answers, QASnowball first divides the document set into several parts $\mathcal{D}_1, \mathcal{D}_2, \ldots, \mathcal{D}_t$ according to the total number of iterations $t$. At the $i$-th iteration, QASnowball automatically annotates the questions and answers for $\mathcal{D}_i$ and generates the dataset $\mathcal{S}_i$, the whole process is given as
\begin{equation*}
\mathcal{S}_i = \cup_{D \in \mathcal{D}_i} \mathcal{G}_D.
\end{equation*}
After obtaining $\mathcal{S}_i$, we update the seed set $\mathcal{S}$ with $\mathcal{S}_i$, and the updated seed set is used to fine-tune the modules of QASnowball. In general, the updating strategy can be to replace $\mathcal{S}$ with $\mathcal{S}_i$ or to merge $\mathcal{S}$ and $\mathcal{S}_i$. Due to our pilot experiments, we merge $\mathcal{S}$ and $\mathcal{S}_i$ to update the seed set in this paper. In fact, more sophisticated strategies can be used here to update the seed set as well, and we leave this for future work. Algorithm~\ref{alg:AOA} shows the iterative bootstrapping process of QASnowball.



==> backup/3_related_work.tex <==
\section{Related Work}
\subsection{Question Answering}
Question Answering (QA) aims to answer the given questions in natural language. Based on the presence of contextual information, QA can be further categorized into two tasks, i.e. machine reading comprehension (MRC) and open-domain QA (ODQA)~\citep{DBLP:journals/corr/abs-2101-00774}. Specifically, MRC requires machines to answer questions based on the given document, while ODQA aims to answer factoid questions without any context. In this paper, we choose the MRC task to examine the effiectiveness of the proposed method, as xxx.
% zz: why we choose the MRC task.
% zz: exsiting models have some drawbacks that can be solved by using QAsnowball?

\subsection{Question Generation and QA Data}

Question Generation (QG) aims to generate questions based on the given document and answers, which has been applied to various tasks, such as data augmentation~\citep{alberti-etal-2019-synthetic} and document retrieval~\citep{DBLP:journals/corr/abs-1904-08375}. Some prior works also leverage question generation to generate QA-pairs, such as PAQ~\citep{lewis-etal-2021-paq} and OceanQA~\citep{}. However, these works use the generated QA-pairs to xxx. While in this paper, we xxx, which can boost the performance of the existing state-of-the-art QA model. 
% zz: say something about the lack of supervised QA data?
% zz: our generated QA-pairs can help the community to build a robust QA system, etc.
 
\subsection{Self-enhanced bootstrapping system}
Snowball was first introduced by \citet{agichtein2000snowball} for relation extractions task. The systems generate extraction patterns as well as new seed tuples which enables an improvement of the quality significantly. More similar bootstrapping systems have been introduced since then, for example, StatSnowball\citep{zhu2009statsnowball} and Neural Snowball\citep{gao2020neural}, both aiming for improving relation extraction through iterations. To the best of our knowledge, we are the first who applied this Snowball-like system in QA-pairs generations and test on many datasets.

% \subsection{Question Generation}
% Questions generation is a task to automatically generate questions from given passages and answers. After its first proposition by \citeauthor{article}, question generations have been a topic of interest for various purposes, such as data augmentation\citep{alberti-etal-2019-synthetic,lewis-etal-2021-paq}. Seldom of them address how to use these data properly for the QA system let alone a bootstrapping pipeline for better generations of the QA-pairs. Similar to our work, OceanQA\citep{fang2020accelerating} and RePAQ\citep{lewis-etal-2021-paq} both contain a pipeline consisting of answer extraction, and question generations and are used in open domain question answering. In contrast, we present a multi-lingual self-enhanced pipeline that contains a QA-pairs filtering process with the state-of-the-art CBQA model. Generated QA-pairs are also proven to be useful for improving a QA system.\citep{yang-etal-2017-semi,dhingra2018simple}

% \subsection{QA-pairs generation}
% An effective and efficient QA-pairs generations pipeline for data augmentation has been a spotlight topic in recent years\citep{lewis-etal-2021-paq,fang2020accelerating}. 
% To the best of our knowledge \citeauthor{DBLP:conf/acl/AlbertiAPDC19} is the first to introduce a simple backbone of the QA-pairs generation pipeline which is similar to our pipeline in one iteration and has proven its effectiveness in the roundtrip consistency process. 
% PAQ\citep{lewis-etal-2021-paq} is currently the largest open-source QA-pairs dataset with a Fusion-in-decoder filter(FiD)\citep{DBLP:conf/eacl/IzacardG21} and a retrieval model RePAQ for answers selection, adversarial data generation\citep{DBLP:conf/emnlp/BartoloTJ0SK21} is also a QA-pair generation pipeline which improves the quality with an adversarial data collection process. We are the first to introduce a snowball-like iterative QA-pair generation pipeline and prove its effectiveness as well as open source a large-scale dataset for both English and Chinese.

% \subsection{Phrase-indexed QA and generative QA-pairs dataset}

% In phrase-indexed QA(PIQA) sysems \citep{seo-etal-2018-phrase,lee-etal-2021-learning-dense}, a neural encoding of an answer span will match with questions according to its possible index. The system is very fast at query time.

% Systems like PAQ/RePAQ and QEDB\citep{https://doi.org/10.48550/arxiv.2207.00630} are related to PIQA, similar to those QA systems. Snowball-QA will have additional computational costs such as on question generations but are more verifiable and highly controllable during our process and eventually help exceed the query time of the QA system.


==> backup/4_method.tex <==

\section{QASnowball}

In this section, we will introduce the details of our iterative bootstrapping framework QASnowball.

\subsection{The Overall Framework}

The main idea of QASnowball is to collect some supervised QA data as a seed set and then automatically generate more QA data based on the seed set. As shown in Figure~\ref{fig:filter}, the overall framework of QASnowball consists of three main modules: an answer extractor, a question generator, and a QA data filter. To achieve the purpose of automatically generating data, three modules work in a pipeline sequentially to generate QA data.

More specifically, given an unlabeled document $d$: (1) \textbf{The answer extractor} is first used to extract the core phrases that are most likely to be answered in the unlabeled document $d$ as candidate answers $\mathcal{A}_d = \{a_d^1, a_d^2, \ldots, a_d^n\}$. (2) \textbf{The question generator} aims to generate the question set $\mathcal{Q}_d = \{q_d^1, q_d^2, \ldots, q_d^n\}$ corresponding to the answer set $\mathcal{A}_d$, by considering both the semantic information of the given document and the candidate answers, where $q_d^i$ is the question corresponding to the candidate answer $a_d^i$. (3) \textbf{The QA data filter} aims to filter out high-quality question-answer pairs from the combinations of the extracted answer set $\mathcal{A}_d$ and the generated question set $\mathcal{Q}_d$. 
The selected question-answer pairs will be combined with the document as the data for training QA models.

The answer extractor, question generator, and QA data filter are first trained on the supervised seed set. Considering the seed set cannot cover sufficient data to train all modules well, QASnowball thus iteratively generates QA data. After each iteration, the newly formed QA data is used to expand the seed set and fine-tune the three modules, and QASnowball goes over the whole process again in the subsequent iterations after finishing fine-tuning the three modules. 

Next, we will briefly introduce the three modules and describe how to make the whole framework iteratively self-enhance.

\subsection{Answer Extractor}

Given a document $d$, the answer extractor aims to identify spans in the document that are likely to be answers to questions. We treat this extraction task as a sequence labeling problem. For each token in $d$, we ask the extractor to determine whether the token is part of a candidate answer, and merge those adjacent tokens that are predicted to be part of answers to form candidate answers.
Specifically, we adopt BERT as the backbone model, which is a typical auto-encoding PLM built on the encoder architecture, and then build a binary classifier based on the backbone to identify whether each token of the input document is part of an answer.
Since the whole process of answer extraction is similar to typical word segmentation and named entity recognition, we will not go into details here. To train the answer extractor, we first use the initial seed set consisting of supervised QA samples, by taking the document and answer of each seed sample as the supervision signal. Then, during the iterative data generation process, the newly generated QA data will be used to further fine-tune the extractor. In order to facilitate the subsequent introduction of our framework, we formalize the extraction process as
\begin{equation}
\small
\mathcal{A}_d = \{a_d^1, a_d^2, \ldots, a_d^n\} = \texttt{AExtractor}(d).
\end{equation}

\subsection{Question Generator}

For the question generator, we select T5~\cite{} as the backbone model, which is a typical generative PLM built based on the encoder-decoder architecture. Specifically, given a document $d$ and a candidate answer $a_d^i$ extracted from $d$, we first add some special tag tokens before and after the span of $a_d^i$ in the document $d$, which can highlight the position of the candidate answer in the document to generate the answer-specific question. For example, given the document ``... It is based in Englewood Cliffs, New Jersey ...'' and the candidate answer ``Englewood Cliffs'', we can add two special tokens (e.g., ``<ANS>'' and ``<ANS/>'') into the document, and then input ``... It is based in <ANS> Englewood Cliffs <ANS/>, New Jersey ...'' into the question generator. By feeding the tagged document into the encoder of the question generator, the decoder of the question generator can output the question corresponding to the document and the answer. To train the question generator, we first use the initial seed set consisting of supervised QA samples, by taking the document and answer of each QA sample in the seed set as input and the answer as the output supervision signal. Then, during the iterative data generation process, the newly generated QA data will be used to further fine-tune the generator, enabling the generator to generate more diverse questions beyond the domain constraints of the initial seed set. Similar to the answer extractor, we formalize the generation process as
\begin{equation}
\small
\mathcal{Q}_d = \{q_d^1, q_d^2, \ldots, q_d^n\} = \texttt{QGenerator}(d, \mathcal{A}_d).
\end{equation}

\subsection{QA Data Filter}

Existing methods usually train a QA model to filter the generated QA data, such as using a MRC model ~\cite{} or a ODQA model ~\cite{} to filter the data. Given a document and its generated question-answer pair, these QA models can evaluate the reasonableness of the answer based on the semantics of the document and the question. The reasonableness scores given by QA models are used to select high-quality generated QA data. Although these methods have achieved promising results, the filtering quality of these methods depends heavily on the quality of the trained QA models, and it is difficult to filter out some correctly generated samples that are judged ambiguous by the QA models themselves, obviously contradicting the purpose of generating QA data to further enhance QA models.

In this paper, we adopt the recently proposed QA model PERT~\cite{} as the backbone of our filter, and we build the data filter based on the ensemble of the backbone model and heuristic rules. Specifically, given the document $d$, the extracted answer $a_d^i$, and the generated question $q_d^i$, we first require the filter backbone to generate an answer $\tilde{a}_d^i$ based on $p_d^i$ and $q_d^i$, without considering $a_d^i$. Then, several heuristic rules are used to select and modify the generated data:
\begin{itemize}
\item if $a_d^i$ does not overlap with $\tilde{a}_d^i$ any more, we discard this example.
\item if $a_d^i$ matches $\tilde{a}_d^i$ exactly, the example $(d, q, a_d^i)$ is finally generated.
\item If $a_d^i$ partially overlaps with $\tilde{a}_d^i$, the example of $(d, q, [a_d^i; \tilde{a}_d^i])$ is finally generated, where $[a_d^i; \tilde{a}_d^i]$ denotes the combination of $a$ and $\tilde{a}$, such as combining ``in Englewood Cliffs'' and ``Englewood Cliffs, New Jersey'' into ``in Englewood Cliffs, New Jersey''.
\end{itemize}
Compared with the existing filtering methods based entirely on QA models, our filter not only ensures the data quality, but also retains some generated data inconsistent with QA models, bring better data diversity. For convenience, we formalize the entire filtering process for the document $d$ as
\begin{equation}
\texttt{Filter}(d, \mathcal{A}_d, \mathcal{Q}_d).
\end{equation}

\subsection{Reseeding and Start next iterations}

To take advantage of more iterations and save the inference time. we first divide the corpus according to our presume iterations number such as 2. And then we only use the first division to generate the QA-pairs and then we use the generated QA-pairs as the updated seed data to retrain the filter model and then adopt the new filter for the second parts of the QA-pairs generation. 

\begin{algorithm}[t]
    \caption{The iterative generation process of QASnowball}
    \label{alg:AOA}
    \renewcommand{\algorithmicrequire}{\textbf{Input:}}
    \renewcommand{\algorithmicensure}{\textbf{Output:}}
    \begin{algorithmic}[1]
        \REQUIRE Seed set $\mathcal{S}$, unlabeled documents $\mathcal{D}$, Total iterations number $t$
        \STATE  Partion unlabeled documents into several parts according to $t$, $\mathcal{D}_{1}, \mathcal{D}_{2}, \ldots, \mathcal{D}_{t}$
        \FOR{$i \in [1, t]$}
            \IF{$i = 0$}
                \STATE Train $\texttt{AExtractor}$, $\texttt{QGenerator}$, and $\texttt{Filter}$ with $\mathcal{S}$.
            \ELSE
                \STATE Fine-tune $\texttt{AExtractor}$, $\texttt{QGenerator}$, and $\texttt{Filter}$ with $\mathcal{S}$.
            \ENDIF
            % \STATE Define the generated data set of the $i$-th iteration 
            \STATE $\mathcal{S}_i = \emptyset$
            \FOR{$d \in \mathcal{D}_{i}$}
                \STATE $\mathcal{A}_d = \texttt{AExtractor}(d)$
                \STATE $\mathcal{Q}_d = \texttt{QGenerator}(d, \mathcal{A}_d)$
                \STATE $\mathcal{S}_i = \mathcal{S}_i \cup \texttt{Filter}(d, \mathcal{A}_d, \mathcal{Q}_d)$
            \ENDFOR
            \STATE $\mathcal{S} = \mathcal{S} \cup \mathcal{S}_i$
        \ENDFOR
        \ENSURE The generated data set of all iterations, $\mathcal{S}_1$, $\mathcal{S}_2$, $\ldots$, $\mathcal{S}_t$
    \end{algorithmic}
\end{algorithm}

% \subsection{SGQ details}

% We obtain 200G raw texts from internet texts, and we first select the highly informative and then cleaned the texts and split them into paragraphs within 1000 words. We first use 5\% percent of the data to generate QA-pairs as iteration 0 data. After we retrain our filter, we then chose 10\% of the raw texts for generating the data of the next iteration. We use the rest of the texts and $filter_{2}$ for generated the final SGQ dataset.


==> backup/5_experiments.tex <==
\section{Experiments}

An Iterative Bootstrapping Framework 


We conduct experiments on the high-resource English scenario and the medium-resource Chinese scenario, and the experimental results show that our generated data can facilitate QA models: (1) training models on the generated data achieves comparable results to using supervised data, and (2) pre-training on the generated data and fine-tuning on supervised data can achieve better performance.
Our system and data will be released to advance further work soon.

\paragraph{Experiment Settings}

For the high-resource English scenario, we conduct experiments on 
SQuAD~\cite{}, TriviaQA-wiki\cite{joshi-etal-2017-triviaqa}, TriviaQA-web\cite{joshi-etal-2017-triviaqa}, and HotpotQA\citep{yang2018hotpotqa}.
Among these datasets, we select SQuAD, TriviaQA-wiki, TriviaQA-web as the seed set to automtically generate large-scale English QA data, and remain HotpotQA to evaluate the transferability of our generated English data, i.e., to evaluate whether our framework can generate some data out of the distribution of the initial seed set.

For the medium-resource Chinese scenario, we conduct experiments on CMRC2018~\cite{cui-emnlp2019-cmrc2018}, DuReader\cite{he-etal-2018-dureader}, SQuAD-zh~\footnote{\url{https://github.com/junzeng-pluto/ChineseSquad/tree/master/squad-zen}}, and DRCD\cite{DBLP:journals/corr/abs-1806-00920}. 
Among these datasets, we select CMRC2018, DuReader, SQuAD-zh as the seed set to automtically generate large-scale Chinese QA data, and remain DRCD to evaluate the transferability of our generated Chinese data.

Since our main focus is to evaluate the quality of our generated data, we conduct both English and Chinese experiements under the machine reading comprehension setting. Under this setting, all answers can be found in documents. Considering that not all of the above datasets are constructed under this setting, we remove all examples in these datasets whose answers are not mentioned in documents. More details about these datasets could be found in our appendix. For the QA model, we select PERT for our expeiments, use different data (including both generated data and supervised data) to train PERT, and .
We use exact match(EM), F1 score as the metrics to evaluate the model prefoance.



\subsection{The Qulaity of }

% \begin{figure*}[htbp]
%   \begin{minipage}{0.45\linewidth}
%     \includegraphics[width=\linewidth]{figs/bar-plot-EM.png}
%     \caption{Zero-shot experiments results on different datasets/}
%   \end{minipage}
%   \begin{minipage}{0.45\linewidth}
%     \includegraphics[width=\textwidth]{figs/bar-plot-f1.png}
%     \caption{Zero-shot experiments results on different datasets}
%   \end{minipage}
%   \begin{minipage}{0.45\textwidth}
%     \includegraphics[width=\textwidth]{figs/bar-plot-EM-en.png}
%     \caption{Zero-shot experiments results on different datasets/}
%   \end{minipage}
%   \hspace{0.05\textwidth}
%   \begin{minipage}{0.45\textwidth}
%     \includegraphics[width=\textwidth]{figs/bar-plot-F1-en.png}
%     \caption{Zero-shot experiments results on different datasets}
%   \end{minipage}
%     \label{fig:zero-shot}
% \end{figure*}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\small
\centering
\begin{tabular}{lllcc}
\toprule
Dataset                   & Shot                & Metric & Seed & Seed+SGQ \\
\midrule
\multirow{6}{*}{HotpotQA} & \multirow{2}{*}{0}  & EM     & 53.1 & 55.3 (+2.2)   \\
                          &                     & F1     & 66.6 & 68.0 (+1.4)   \\
\cmidrule{2-5}
                          & \multirow{2}{*}{8}  & EM     & 53.1 & 55.7 (+2.6)   \\
                          &                     & F1     & 66.6 & 68.6 (+2.0)   \\
\cmidrule{2-5}
                          & \multirow{2}{*}{32} & EM     & 55.0 & 56.5 (+1.5)   \\
                          &                     & F1     & 68.9 & 69.6 (+0.7)   \\
\midrule
\multirow{6}{*}{DRCD}     & \multirow{2}{*}{0}  & EM     & 71.8 & 74.3 (+2.5)   \\
                          &                     & F1     & 85.1 & 86.4 (+1.3)   \\
\cmidrule{2-5}
                          & \multirow{2}{*}{8}  & EM     & 73.3 & 74.7 (+1.4)   \\
                          &                     & F1     & 85.9 & 86.6 (+0.7)   \\
\cmidrule{2-5}
                          & \multirow{2}{*}{32} & EM     & 74.9 & 76.3 (+1.4)   \\
                          &                     & F1     & 86.6 & 87.4 (+0.8)   \\
\bottomrule
\end{tabular}
\caption{\label{filter-score-comparison}
Zero-shot and Fine-tune experiments results(\%) for English corpus. 1M data is the 1 million data generated by our pipeline through the Wikipedia articles.
}
\end{table}



% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
\small
\centering
\begin{tabular}{l|cc|cc|cc|cc|cc}
\toprule
\multirow{2}{*}{Dataset} & \multicolumn{2}{c|}{CMRC} & \multicolumn{2}{c|}{SQuAD-ZH} & \multicolumn{2}{c|}{DuReader} & \multicolumn{2}{c|}{DRCD*} & \multicolumn{2}{c}{Average} \\
                         & EM          & F1         & EM            & F1           & EM            & F1           & EM          & F1         & EM         & F1         \\
\toprule
$\text{SGQ}_1$  & 67.2        & 86.8       & 55.5          & 73.3         & 65.8          & 81.8         & 67.8        & 83.4       & 64.1     & 81.3     \\
$\text{SGQ}_2$  & 71.6        & 88.0         & 57.8          & 74.8         & 70.9          & 83.7         & 70.5        & 84.7       & 67.7       & 82.8       \\
$\text{SGQ}_1-\text{SGQ}_2$ & 33.4        & 78.5       & 40.7          & 66.0           & 34.1          & 72.5         & 45.6        & 73.2       & 38.5      & 72.6      \\
$\text{SGQ}_2-\text{SGQ}_1$ & 70.9        & 85.5       & 41.9          & 66.3         & 66.3          & 79.9         & 68.4        & 81.1       & 61.9     & 78.2      \\
\bottomrule
\end{tabular}
\caption{\label{zero-shot}
A study on why model pre-trained with the former iteration data can not perform better than that with the next iteration in In-domain Fine-tune. We first take apart the 470k filtered data in the 2nd iteration into two parts. One part is $iter_{0} \cap iter_{1}$, this part was not updated during the second iteration. Another part is the remaining updated data. $iter_{0-diff}$ is the updated data's original data in the 1st iteration, $iter_{1-diff}$ is the updated data in the 2nd iteration.
}
\end{table*}




\subsection{Analysis on Few-shot experiments}

\textbf{Results}  To examine the quality of our SGQ dataset, we first pre-train the PERT model for question-answering tasks by predicting the answer spans in the given passages. We first use seed dataset to pre-trained PERT and get $PERT_{seed}$. We then use 1 million QA-pairs from our SGQ dataset and get $PERT_{seed+1M}$, and then test its few-shot and zero-shot ability on multiple datasets, including CMRC2018, DuReader, DRCD, and SQuAD-Zh. We observe that our zero-shot test for the $PERT_{seed+1M}$ model still shows a considerably good result on HotpotQA and DRCD in Table 1. 

Figure 3 and Figure 4 also show that the zero-shot setting from the model trained on our SGQ datasets already shows high quality compared with the fine-tuned models. We see that our zero-shot model performs even better in the F1 rate on the CMRC2018 dataset, that is because the PERT model is already pre-trained on the CMRC training set.


\begin{table*}[t]
\small
\centering
\begin{tabular}{c|cc| cc| cc| cc| cc}
\toprule
\multirow{2}{*}{SGQ Amount} & 
\multicolumn{2}{c|}{{CMRC}} &
\multicolumn{2}{c|}{{SQuAD-zh}} &
\multicolumn{2}{c|}{{DuReader}} &
\multicolumn{2}{c|}{{DRCD}} & 
\multicolumn{2}{c}{\textbf{Average}}\\
& EM & F1 & EM & F1 & EM & F1 & EM & F1 & EM & F1\\ 
\midrule
0.0M & 69.4 & 86.0  & 59.6 & 76.1 & 73.2 & 85.3 & 88.7 & 93.9  & 72.8 & 85.3\\
\midrule
% & 10k & 71.0 & 86.7  & 59.9 & 76.5 & 88.4 & 93.5 & 73.1 & 85.3 & 73.1 & 85.5\\
0.1M & \textbf{73.6} & 88.3  & 60.2 & 76.6 & 74.0 & 86.3 & 88.1 & 93.5  & 74.0 & 86.2\\
0.5M & 72.8 & 89.3  & 60.6 & 77.0 & 75.0 & 86.6 & 89.3 & 94.3  & 74.5 & 86.8\\
1.0M & 73.3 & 89.5  & 60.3 & 76.7 & \textbf{76.1} & \textbf{86.9} & \textbf{89.6} & \textbf{94.3}  & 74.8 & 86.9\\
5.0M & 73.4 & \textbf{90.1} & \textbf{60.8} & \textbf{77.4} & 75.7 & 86.8 & 89.5  & \textbf{94.3}  & \textbf{74.9} & \textbf{87.2}\\
\bottomrule
\end{tabular}
\caption{\label{data-amount}
Pretrain PERT with increasing amount of our data, then fine-tune and test on each benchmark's train set and development set. 0 means fine-tune directly on individual training sets without pretraining with our data.
}
\end{table*}



\begin{table*}[t]
\small
\centering
\begin{tabular}{p{11cm}|p{3cm}}
\toprule
Passage & Question \\
\midrule
\begin{CJK}{UTF8}{gbsn}探讨电视胸腔镜辅助小切口手术(vamt)在自发性气胸治疗中的应用价值。\colorbox{green}{方法是}\colorbox{yellow}{于患侧腋中线第6或第7肋间置入胸腔镜套管} \colorbox{green}{，在靠近病变位置做长约5~8cm切口经肋间进胸(多在腋} \colorbox{green}{前线或腋中线第4~5肋)，使用普通手术器械与胸腔镜手术} \colorbox{green}{器械，在胸腔镜和直视下进行操作。}\end{CJK}
\textbf{Translation}: Discussion of small incision hand assisted by video-assisted thoracoscopic Application value of surgery in the treatment of spontaneous pneumothorax value. Methods A thoracoscopic cannula was placed in the 6th or 7th intercostal space on the midaxillary line of the affected side, make an incision about 5-8cm long near the lesion and enter the chest through the intercostal area (mostly in the axilla) 4th to 5th ribs on the front line or midaxillary line), using common surgical instruments and thoracoscopic surgery Instruments, operated under thoracoscopic and direct vision. & 
\begin{CJK}{UTF8}{gbsn}
电视胸腔镜辅助小切口手术的方法是什么?
\end{CJK}
What is the method of video-assisted thoracoscopic small incision surgery?
\\
\hline

\begin{CJK}{UTF8}{gbsn}移动学习逐渐成为一种趋势，而\colorbox{yellow}{移动学习资源开发}\colorbox{red}{是开展移动学习至关重要}的环节。文章详细分析了目前移动学习资源开发中流行的几种移动开发平台及开发工具，并针对其是否适合移动学习资源开发而进行了评价总结\end{CJK}

\textbf{Translation}:Mobile learning has gradually become a trend, and the development of mobile learning resources is a crucial link in the development of mobile learning. The article analyzes in detail several popular mobile development platforms and development tools in the development of mobile learning resources, and evaluates whether they are suitable for the development of mobile learning resources. & 
\begin{CJK}{UTF8}{gbsn}
移动学习资源有哪些环节?
\end{CJK}
What are the links of mobile learning resources?
\\
\bottomrule
\end{tabular}
\caption{\label{filter-score-comparison}
Examples of iter1 and iter2 answers. Green color box texts indicates iteration 2 extracted answer, red color box texts indicate the iteration 1 answer, yellow color box texts indicates the overlapping texts. Translation is done by google Translate.
}
\end{table*}

\begin{figure}[htbp]
  \begin{minipage}{0.21\textwidth}
    \includegraphics[width=\textwidth]{figs/bar-plot-EM.pdf}
    \caption{Comparison between SGQ and supervised on different datasets/}
  \end{minipage}
  \hspace{0.05\textwidth}
  \begin{minipage}{0.21\textwidth}
    \includegraphics[width=\textwidth]{figs/bar-plot-f1.pdf}
    \caption{Comparison between SGQ and supervised on different datasets/}
  \end{minipage}
\end{figure}

\begin{figure}[htbp]
  \begin{minipage}{0.21\textwidth}
    \includegraphics[width=\textwidth]{figs/bar-plot-EM-en.pdf}
    \caption{Comparison among PAQ, SGQ and supervised on different datasets}
  \end{minipage}
  \hspace{0.05\textwidth}
  \begin{minipage}{0.21\textwidth}
    \includegraphics[width=\textwidth]{figs/bar-plot-F1-en.pdf}
    \caption{Comparison among PAQ, SGQ and supervised on different datasets}
  \end{minipage}
\end{figure}

\subsection{Experiments on the data quality in different iterations}
To further analyze the iterative process of Snowball-QA pipeline, we test our model on multiple datasets with different combinations of our SGQ data in different iterations. We still chose PERT as our baseline model. We also compares the results by separately pre-train the model with different iterations of data and a mixture of SGQ data from two iterations.

We first observe that about 70\% percent of data are exactly the same between iteration 0 and iteration 1 filtered datasets. We then compare the different answer spans for the same questions within iteration 0 and iteration 1.

Table 2 demonstrates the usefulness of our iterative Snowball-QA pipeline. And the data quality will increase as the iterative process continue. Here we adopt three settings for representing the different types of data generated by our model. \textbf{$Iter_{0}$} represent the QA-pair data generated by our pipeline in the first iteration, \textbf{$Iter_{1}$} refers to the QA-pair data generated by our pipeline during the second iteration, and \textbf{$Iter_{0,differed}$} and \textbf{$Iter_{1,differed}$} refers to the different QA-pairs when processing the same text by the filter in the first iteration and the second one correspondingly.

We see that the PERT model pre-trained with the \textbf{$Iter_{0,differed}$} data perform surprising bad on each dataset, and PERT trained with \textbf{$Iter_{1,differed}$} are much higher and even comparable with PERT pre-trained with \textbf{$Iter_{0}$} which has much more data. It demonstrates that the quality of the data in the second iteration is much higher than the first iteration. Results in Table 3 also show that our filter in the second iteration performs much better than the filter in the first iteration.

We thus conclude that 1)our snowball pipeline can greatly improve data quality, and 2) we can utilize both the filter0 and filter1 by intersecting the data filtered by them which has shown better results.

\subsection{Experiments on the intersection between iterations}

Table 3 shows the intersection dataset results between SGQ-0 and SGQ-1

\subsection{Experiments on the human evaluation}
For the human evaluation part, We randomly chose 200 QA-pairs each from the first and second iterations, where they have the same texts and questions but with different answers. Comparing the QA-pairs at least one of them is valid, the QA-pairs from the second iteration is 75.3\% better by chance. We then randomly chose 100 QA-pairs each from the first and the second iteration, in the first iteration, 73\% of the QA-pairs are valid which means they are correct by human standards, and 82\% of the QA-pairs are valid in the second iteration. This demonstrates the effectiveness of our QAsnowball framework that we can iteratively improve the quality of our generated QA-pairs.

In the human comparison results, we observe that both the answers of iteration 0 and iteration 1 are valid, iteration 1's answers are 75\% better which proves the effectiveness of our snowball self-enhanced pipeline.  



\subsection{Case Study}
In Table 4, We also observe that iteration 1 answers are not only able to extract answer spans that are supposed to be long but also able to answer the questions in a more succinct way. 


% In Table 4, we can see that after retraining from the first iteration, our QASnowball is able to tackle longer answers which is more accurate than the original short answer span. We believe this is because 1) the post-process from our answer extraction enables our pipeline to extract longer and more complex answers and 2) the combination process by our filter enables our system to compare and complete the answer more thoroughly and enables the system to generate longer answer span which is more accurate.

==> backup/6_analysis.tex <==
\section{Analysis}

\subsection{why do we not retrain the answer extractor and question generator in later iterations}
    This is the trade-off we make for our overall pipeline. We found that the retraining answer extractor and question generator parts are highly time-consuming and didn't improve the final data quality lot. In addition, the pipeline won't change any data the question generator had generated, so it would be adding no extra ability for the question generator to generate new types of questions or higher quality questions. Our answer filter is also able to tackle the problem meet in the question generation and extraction part by filtering the unqualified results or changing them.
    
\subsection{Why would the system be better through iterations of training?}

The Key component for ensuring the quality of our generated data is the filter. The idea of our pipeline is to cor-ordinate three parts of our framework by mitigating the bias between different parts and increasing the robustness of our system through iterations. By 1 or 2 iterations of retraining on the filter, we demonstrate the filter would be able to become more familiar with the raw texts since the text style might be very different from the pre-training texts. And by filtering the higher-quality data with our filter, the filter can extract the answers better fit into the metric. Another reason is that high-quality seed data is rare, and through the framework of Snowball-QA, it's equal to the data augmentation process with similar quality as the seed data.
 
\subsection{Reasons for Not Using Score for Filtering}
A classical self-training data generation approach uses the predicted score of a filtering model to filter the dirty data. However, data generated in this way will be limited by the capabilities of the filtering model. For example, some data are given a low score by the filtering model, while they should probably be treated as strong negative data. We replace the score filtering of rule-based approaches and a filter strategy. In answer generation, we use answer post-processing to initially correct the answers; in question generation, we keep all the questions; and in the final QA-pair filtering, we use rule-based filtering based on the filter model. We aim to increase the amount of data while introducing such strong negative examples to enhance the performance of the model.% We experimentally validate our idea that the rule base filtered data performs comparably or better than the scoring base filtered data in the Chinese benchmarks.

==> backup/7_conclusion.tex <==
\section{Conclusion}

In this paper, we propose QASnowball, a novel framework that can continually generate data with higher quality and larger scale. We conduct our experiments based on the main Machine Reading Comprehension Benchmarks, in both Chinese and English. Results show that our auto-generated data can enable PLM with stable QA ability, and is comparable to the human-annotated or supervised data. Evaluations on the Chinese MRC benchmarks demonstrate the data could bring significant improvement when used as pre-training data. Further analysis proves the effectiveness of the snowball process, thus we can constantly improve the QA ability and benchmarks' performance of PLM with our deeper iterations' data. 

In the future: we will further explore the following directions:

(1) Chain of thought\citep{wei2022chain} type of QA data generation from raw text. 

(2) Exploring the limits of the data quality improvement when the iterations continue to increase and showing more interpretability of how this iterative process actually helps each part of the model.

==> backup/8_ethical.tex <==
\section{Ethical Consideration}
Our raw texts are collected from the internet, and as though we have cleaned the data to a large extent, we can not ensure all of our text sources are safe. So, we will only provide limited access to our dataset for research purposes only, and we do not foresee any risks associated with the use of our data at this point.


==> backup/9_acknowledge.tex <==
\section*{Acknowledgements}
This work has been supported by the Beijing Academy of Artificial Intelligence and the research fund of Tsinghua University Natural Language Processing Lab. We would also like to thank the OpenBMB team for some great advice and feedback.
